Emergence of simple and complex contagion dynamics from weighted belief networks

Social contagion is a ubiquitous and fundamental process that drives individual and social changes. Although social contagion arises as a result of cognitive processes and biases, the integration of cognitive mechanisms with the theory of social contagion remains an open challenge. In particular, studies on social phenomena usually assume contagion dynamics to be either simple or complex, rather than allowing it to emerge from cognitive mechanisms, despite empirical evidence indicating that a social system can exhibit a spectrum of contagion dynamics -- from simple to complex -- simultaneously. Here, we propose a model of interacting beliefs, from which both simple and complex contagion dynamics can organically arise. Our model also elucidates how a fundamental mechanism of complex contagion -- resistance -- can come about from cognitive mechanisms.

==> Belief_Network_paper/ScienceAdv/subparts/markov_complex.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{|c|c|}
        \hline
        \textbf{ID} & \textbf{Belief Network State} \\
        \hline
        0 & $\{-1, -1, 1\}$ \\
        1 & $\{-1, -0.5, 1\}$ \\
        2 & $\{-0.5, -1, 1\}$ \\
        3 & $\{-0.5, 0, 1\}$ \\
        4 & $\{-0.5, 1, 1\}$ \\
        5 & $\{-1, 0, 1\}$ \\
        6 & $\{0, -1, 1\}$ \\
        7 & $\{0.5, -1, 1\}$ \\
        8 & $\{-1, 0.5, 1\}$ \\
        9 & $\{-1, 1, 1\}$ \\
        10 & $\{0, 0.5, 1\}$ \\
        11 & $\{0, 1, 1\}$ \\
        12 & $\{0, -0.5, 1\}$ \\
        13 & $\{1, 0.5, 1\}$ \\
        14 & $\{1, 1, 1\}$ \\
        15 & $\{1, 0, 1\}$ \\
        16 & $\{0.5, 1, 1\}$ \\
        17 & $\{0.5, 0, 1\}$ \\
        18 & $\{1, -0.5, 1\}$ \\
        19 & $\{1, -1, 1\}$ \\
        \hline
    \end{tabular}
    \caption{\textbf{All the states the hub can transition to in scenario 2 of the star graph setting}. Each state is mapped to a  unique ID. }
    \label{tab:states_scenario2}
\end{table}

\begin{table}[htbp]
    \centering
    \begin{minipage}{0.2\linewidth}
        % \caption*{Part 1}
        \begin{tabular}{|c|c|c|}
            \hline
            \textbf{SID} & \textbf{DID} & \textbf{TP} \\
            \hline
            0 & 0 & $u + 3v$ \\
            0 & 1 & $u$ \\
            0 & 2 & $u$ \\
            1 & 0 & $v$ \\
            1 & 1 & $u + 2v$ \\
            1 & 5 & $u$ \\
            1 & 12 & $u$ \\
            2 & 0 & $v$ \\
            2 & 2 & $u + 2v$ \\
            2 & 3 & $u$ \\
            2 & 6 & $u$ \\
            3 & 2 & $v$ \\
            3 & 3 & $u + v$ \\
            3 & 4 & $u$ \\
            3 & 5 & $v$ \\
            3 & 15 & $u$ \\
            4 & 2 & $v$ \\
            4 & 4 & $2u + v$ \\
            4 & 9 & $v$ \\
            4 & 14 & $u$ \\
        \hline
        \end{tabular}
    \end{minipage}
    \hspace{0.05\linewidth} % Adjust the horizontal space between the tables
    \begin{minipage}{0.2\linewidth}
        % \caption*{Part 2}
        \begin{tabular}{|c|c|c|}
            \hline
            \textbf{SID} & \textbf{DID} & \textbf{TP} \\
            \hline
            5 & 0 & $v$ \\
            5 & 5 & $2v + u$ \\
            5 & 8 & $u$ \\
            5 & 17 & $u$ \\
            6 & 0 & $v$ \\
            6 & 6 & $u + 2v$ \\
            6 & 7 & $u$ \\
            6 & 9 & $u$ \\
            7 & 0 & $v$ \\
            7 & 6 & $u + 2v$ \\
            7 & 16 & $u$ \\
            7 & 19 & $u$ \\
            8 & 0 & $v$ \\
            8 & 8 & $u + 2v$ \\
            8 & 9 & $u$ \\
            8 & 14 & $u$ \\
            9 & 0 & $v$ \\
            9 & 9 & $2u + 2v$ \\
            9 & 14 & $u$ \\
            10 & 6 & $v$ \\
        \hline
        \end{tabular}
    \end{minipage}
    \hspace{0.05\linewidth} % Adjust the horizontal space between the tables
    \begin{minipage}{0.2\linewidth}
        % \caption*{Part 3}
        \begin{tabular}{|c|c|c|}
            \hline
            \textbf{SID} & \textbf{DID} & \textbf{TP} \\
            \hline
            10 & 8 & $u$ \\
            10 & 10 & $u + v$ \\
            10 & 11 & $u$ \\
            10 & 13 & $u$ \\
            11 & 4 & $v$ \\
            11 & 11 & $2u + v$ \\
            11 & 12 & $v$ \\
            11 & 14 & $u$ \\
            12 & 1 & $v$ \\
            12 & 6 & $v$ \\
            12 & 11 & $u$ \\
            12 & 12 & $u + v$ \\
            12 & 18 & $u$ \\
            13 & 10 & $v$ \\
            13 & 13 & $2u + v$ \\
            13 & 14 & $u$ \\
            13 & 15 & $v$ \\
            14 & 13 & $v$ \\
            14 & 14 & $3u + v$ \\
            14 & 16 & $v$ \\
        \hline
        \end{tabular}
    \end{minipage}
    \hspace{0.05\linewidth} % Adjust the horizontal space between the tables
    \begin{minipage}{0.2\linewidth}
        % \caption*{Part 4}
        \begin{tabular}{|c|c|c|}
            \hline
            \textbf{SID} & \textbf{DID} & \textbf{TP} \\
            \hline
            15 & 3 & $v$ \\
            15 & 14 & $u$ \\
            15 & 15 & $2u + v$ \\
            15 & 18 & $v$ \\
            16 & 11 & $v$ \\
            16 & 14 & $u$ \\
            16 & 16 & $2u + v$ \\
            16 & 17 & $v$ \\
            17 & 5 & $v$ \\
            17 & 7 & $u$ \\
            17 & 14 & $u$ \\
            17 & 15 & $u$ \\
            17 & 16 & $u + v$ \\
            18 & 1 & $v$ \\
            18 & 14 & $u$ \\
            18 & 18 & $2u + v$ \\
            18 & 19 & $v$ \\
            19 & 0 & $v$ \\
            19 & 14 & $u$ \\
            19 & 19 & $2u + 2v$ \\
        \hline
        \end{tabular}
    \end{minipage}
    \caption{\textbf{Transition Probabilities (TIP) from Source State (SID) to Destination State (DID) for Scenario 2 in the star graph setting}. Missing SID-DID combinations have a TP of 0.}
    \label{tab:scenario2_transitions}
\end{table}

==> Belief_Network_paper/ScienceAdv/subparts/meafield_sir.tex <==
Here is our analytical evidence that supports the lack of a regime of optimal network modularity in simple contagion.

Consider a susceptible-infected-recovered (SIR) model---a quintessential model of simple contagion. 
Let us explore the macroscopic dynamics of this model on the network with two communities using a mean-field approximation similar to the setup in~\citeauthor{nematzadeh2014optimal}[31]. 
% ~\cite{nematzadeh2014optimal}.

Let us call the two communities as $A$ and $B$. 
Let $\Omega$ be the probability that a specific neighbor of an individual in $A$ is in $B$. 
Let $S_{A(B)}, I_{A(B)}, \eta_{A(B)}$ be the fraction of the susceptible, infected, and recovered individuals respectively, in community $A(B).$
The fraction of individuals in each of these compartments then evolve according to the following dynamical equations:
\begin{equation}~\label{eq:s}
    \frac{\partial S_{A(B)}}{\partial t} = -\beta[(1-\Omega) I_{A(B)} + \Omega I_{B(A)}]S_{A(B)},
\end{equation}
\begin{equation}~\label{eq:i}
    \frac{\partial I_{A(B)}}{\partial t} = \beta[(1-\Omega) I_{A(B)} + \Omega I_{B(A)}] - \gamma I_{A(B)},
\end{equation}
\begin{equation}~\label{eq:eta}
    \frac{\partial \eta_{A(B)}}{\partial t} = \gamma I_{A(B)},
\end{equation}
where $\beta$ is a the transmission rate between susceptible and infected individuals and $\gamma$ is the spontaneous recovery rate of infected individuals.   

Solving this system of equations based on the initial conditions that a fraction $\rho_0$ of individuals in $A$ are infected, i.e $S_A(0) = 1-\epsilon,$ $I_A(0) = \epsilon,$ $\eta_A(0) = 0$, and $S_B(0) = 1,$ $I_B(0) = 0,$ $\eta_B(0) = 0$, the fraction of recovered individuals (end state of the system since recovered individuals don't go back to being susceptible). 
At $t=\infty$, $\eta_A(\infty)$ and $\eta_B(\infty)$ can be derived as follows,

From Eq.~\ref{eq:eta},
\begin{equation}
    \int_0^{\infty}\frac{\partial\eta_A}{\partial t}dt = \eta_A(\infty) - \eta_B(0) = \eta_A(\infty) = \gamma\int_0^{\infty}I_A(t)dt~\label{eq:eta_sol}
\end{equation}

From Eqs.~\ref{eq:s} and~\ref{eq:eta_sol},
\begin{equation}~\label{eq:s_sol}
    -\frac{\gamma}{\beta}\int_0^{\infty}\frac{1}{S_A}\frac{\partial S_A}{\partial t}dt = (1 - \Omega)\gamma\int_0^\infty + \Omega\gamma\int_0^{\infty}I_B(t)dt = (1 - \Omega)\eta_A(\infty) + \Omega\eta_B(\infty).
\end{equation}

From the LHS of Eq.~\ref{eq:s_sol}
\begin{equation}
    -\frac{\gamma}{\beta}\int_0^{\infty}\frac{1}{S_A}\frac{\partial S_A}{\partial t}dt = -\frac{\gamma}{\beta}ln\frac{S_A(\infty)}{ S_A(0)} = -\frac{\gamma}{\beta}ln\frac{1-\eta_A(\infty)}{1-\rho_0} = (1 - \Omega)\eta_A(\infty) + \Omega\eta_B(\infty).
\end{equation}

Therefore, 
\begin{equation}
    \eta_A(\infty) = 1- (1-\rho_0)e^{-\frac{\beta}{\gamma}[(1-\Omega)\eta_A(\infty) + \Omega\eta_B(\infty)]}
\end{equation}

Similarly, based on the condition that $\eta_B = 0$,
\begin{equation}
    \eta_B(\infty) = 1 - e^{-\frac{\beta}{\gamma}[(1-\Omega)\eta_B(\infty) + \Omega\eta_A(\infty)]}
\end{equation}  

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth, trim={0 3in 0 3in}]{ScienceAdv/SIR_meanfield.pdf}
    \caption{\textbf{Simple contagion setting does not show the optimal modularity behavior.} The total fraction of recovered individuals ($\eta_A(\infty) +\eta_B(\infty)$; range of [0,2])) in the mean field setup as probability ($\Omega$) of cross connection between two communities in the stochastic block model setup increases for different initial fraction of infected individuals ($\rho_0$). $\gamma = \beta = 1$.}\label{fig:sir_meanfield}
\end{figure}


==> Belief_Network_paper/ScienceAdv/subparts/sbm_vary_alpha_beta.tex <==
\begin{figure}[!htb]
    % \centering
    \includegraphics[width=1\textwidth, trim={0 0in 0 0in}]{ScienceAdv/optimal_modularity_varyingalphabeta_dualstable_N100_M1500_normalscale0.2_10ensembles.pdf}
    \caption{\textbf{The presence of optimal modularity behavior for different values of model parameters---$\alpha$, and $\beta$}. No diffusion (dark blue), local diffusion in the seed community (green), and global diffusion (yellow). $N=100, M=1500, \sigma=0.2, 10 $ ensembles. }\label{fig:om_varying_alphabeta}
\end{figure}

==> Belief_Network_paper/ScienceAdv/subparts/star_vary_alpha_beta.tex <==
\begin{figure}[!htb]
    % \centering
    \hspace*{-1.5cm}
    \includegraphics[width=1.2\textwidth, trim={0 1in 0 1in}]{ScienceAdv/stargraph_unstable_dualstable_N40_normalscale0.2_ensembles50_batches10_nofocalegde_fixedallneigbhors.pdf}
    \caption{\textbf{The probability that the hub changes to the new belief system exhibits the characteristic behaviors of simple (orange) and complex (blue) contagion for a range of model parameters---$\alpha$ and $\beta$}. The probability is calculated by running the simulation 50 times and calculating the proportion of times the hub `flipped.' Error bars, indicating standard deviation, are then obtained by repeating this process 10 times. \(N=40, M=39,\sigma=0.2\).}\label{fig:varying_alphabeta}
\end{figure}

==> Belief_Network_paper/ScienceAdv/subparts/star_vary_sigma.tex <==
\begin{figure}[!htb]
    % \centering
    \hspace*{-1.5cm}
    \includegraphics[width=1.2\textwidth, trim={0 2.5in 0 3in}]{ScienceAdv/stargraph_unstable_dualstable_N40_ensembles50_batches10_nofocalegde_neighborsfixed_varyingsigma.pdf}
    \caption{\textbf{The probability that the hub changes to the new belief system exhibits the characteristic behaviors of simple (orange) and complex (blue) contagion for different values of $\sigma$}. The probability is calculated by running the simulation 50 times and calculating the proportion of times the hub `flipped.' Error bars, indicating standard deviation, are then obtained by repeating this process 10 times. \(N=40, M=39\)}\label{fig:varying_sigma}
\end{figure}

==> Belief_Network_paper/ScienceAdv/subparts/ws_complex.tex <==
\begin{figure}[!htb]
    % \centering
    \includegraphics[width=1\textwidth, trim={0 1in 0 0in}]{ScienceAdv/dualstable_ws_N100_averagek10_ensembles1_zealotsfixed.pdf}
    \caption{\textbf{The time evolution of the fraction of stable individuals of the type $\{+1,+1,+1\}$ in Scenario 2 of the Watts-Strogatz network setting.} We see a rich range of behaviors. In case of $\rho_0=0.06$, we see that a clustered network structure (Watts Strogatz with rewiring probability $p=0$, blue curve) facilitates the contagion more than a random network structure (Watts Strogatz with rewiring probability $p=1$, orange curve) while in other cases it appears that a random network structure facilitates the contagion more than a highly clustered network structure. The horizontal green line indicates $\rho_0$. N=100, $\bar{k}=10, \sigma=0.2$. Curves are obtained from averaging $3$ ensembles for all subplots except those between $\rho_0=0.06, \rho=0.11$ (included) which is an average of 10 ensembles to save computational time.}\label{fig:wattstrogatz_complex}
\end{figure}

==> Belief_Network_paper/ScienceAdv/subparts/ws_complex_avk5.tex <==
\begin{figure}[!htb]
    % \centering
    \includegraphics[width=1\textwidth, trim={0 1.5in 0 0in}]{ScienceAdv/dualstable_ws_N100_averagek5_ensembles1_zealotsfixed.pdf}
    \caption{\textbf{The time evolution of the fraction of stable individuals of the type $\{+1,+1,+1\}$ in Scenario 2 of the Watts-Strogatz network setting.} We see a rich range of behaviors. In the case of $\rho_0=0.06$, we see that a clustered network structure (Watts Strogatz with rewiring probability $p=0$, blue curve) facilitates the contagion more than a random network structure (Watts Strogatz with rewiring probability $p=1$, orange curve) while in other cases it appears that a random network structure facilitates the contagion more than a highly clustered network structure. The horizontal green line indicates $\rho_0$. N=100, $\bar{k}=5, \sigma=0.2$. Curves are obtained from averaging $2$ ensembles for all subplots.}\label{fig:wattstrogatz_complex_k5}
\end{figure}

==> Belief_Network_paper/ScienceAdv/subparts/ws_simple.tex <==
\begin{figure}[!htb]
    % \centering
    \includegraphics[width=1\textwidth, trim={0 1.5in 0 0in}]{ScienceAdv/unstable_ws_N100_averagek10_ensembles1_zealotsfixed.pdf}
    \caption{\textbf{The time evolution of the fraction of stable individuals of the type $\{+1,+1,+1\}$ in Scenario 1 of the Watts-Strogatz network setting.} We see that a random network structure (Watts Strogatz with rewiring probability $p=1$, orange curve) facilitates the contagion more than a highly clustered network structure (Watts Strogatz with rewiring probability $p=0$, blue curve). The horizontal green line indicates $\rho_0$. N=100, $\bar{k}=10, \sigma=0.2, 2$ ensembles.}\label{fig:wattstrogatz_simple}
\end{figure}
